An improved isomorphism test for bounded-tree-width graphs

We give a new fpt algorithm testing isomorphism of $n$-vertex graphs of tree width $k$ in time $2^{k\operatorname{polylog} (k)}\operatorname{poly} (n)$, improving the fpt algorithm due to Lokshtanov, Pilipczuk, Pilipczuk, and Saurabh (FOCS 2014), which runs in time $2^{\mathcal{O}(k^5\log k)}\operatorname{poly} (n)$. Based on an improved version of the isomorphism-invariant graph decomposition technique introduced by Lokshtanov et al., we prove restrictions on the structure of the automorphism groups of graphs of tree width $k$. Our algorithm then makes heavy use of the group theoretic techniques introduced by Luks (JCSS 1982) in his isomorphism test for bounded degree graphs and Babai (STOC 2016) in his quasipolynomial isomorphism test. In fact, we even use Babai's algorithm as a black box in one place. We also give a second algorithm which, at the price of a slightly worse running time $2^{\mathcal{O}(k^2 \log k)}\operatorname{poly} (n)$, avoids the use of Babai's algorithm and, more importantly, has the additional benefit that it can also used as a canonization algorithm.

==> articles/aut-group.tex <==
\section{The structure of the automorphism group}\label{sec:aut:group}

  In this section, we study the automorphism groups of graphs of
  bounded tree width. Our first result states that the automorphism
  groups of graphs of tree width at most $k$ can be
  formed from the automorphism groups of $k$-basic graphs of tree width at
  most $k$ by (repeatedly) taking direct products and wreath
  products with a symmetric top group. This underlines once more the central role of
  the $k$-basic graphs, which we already observed in the previous
  sections. 

  Let $\Phi_k$ be the class of all automorphism groups of $k$-basic
  graphs of tree width at most $k$. It follows from the results of the
  previous section that we can put these groups into the class
  $\Gammak$ by fixing a single vertex. % This significantly
  % restrict the class of groups in $\Phi_k$
  % and it is the foundation of our canonization algorithm in the
  % following section. Recall that a group is in $\Gammak$ if all
  % non-Abelian composition factors are subgroups of the symmetric group
  % $\sym(k)$. 
  We prove an even stronger restriction on the non-Abelian
  composition factors of groups in $\Phi_k$: they are $\ZZ_p^2$-free
  for all primes $p>k$. 
It follows that the non-Abelian
  composition factors of automorphism groups of graphs of tree width
  at most $k$ are either alternating groups or $\ZZ_p^2$-free
  for all primes $p>k$. 
% Our goal is to describe the automorphism groups
% of graphs with tree width $k$.

% %\begin{conj}[\cite{babai1994automorphism}]
% %For any graph $G$ not having $X$ as a minor
% %the automorphism group $\aut(G)$ is Abelian or non-simple
% %or is one of finitely many exceptions.
% %\end{conj}
% \begin{conj}[\cite{MR633647}]
% Let~$\mathcal{C}$ be a graph class excluding a fixed minor. 
% Then there is a finite set of simple groups~$M_{\mathcal{C}}$ such that 
% for every graph $G\in \mathcal{C}$ every non-Abelian composition factor
% of~$\aut(G)$ is alternating or a member~$M_{\mathcal{C}}$.
% \end{conj}

% To investigate this conjecture for graphs of tree width at most~$k$ we first
% argue that it is sufficient to analyze~$k$-improved clique separator free
% graphs of tree width at most $k$.
% We define $\Phi_k$ as the class of groups
% isomorphic to the automorphism group of a (finite) $k$-improved
% graph of tree width at most $k$ that
% does not have any separating cliques.

We need to introduce two further class of groups derived from
$\Phi_k$. We let~$\Phi_k^{\leq}$ be the class of groups that are
isomorphic to a subgroup of some group in~$\Phi_k$.
Note that every subgroup of~$\sym(k)$ is in~$\Phi_k^{\leq}$ since~$\sym(k)$ is
in $\Phi_k$. We let~$\Psi_k$ be the smallest class of groups that
contains $\Phi_k^{\leq}$ and all symmetric groups and is closed under
taking direct products and wreath products.

% with the following properties:
% \begin{itemize}
% \item $\Phi_k^{\leq}\subseteq \Psi_k$ 
% %\item Every subgroup of~$S_k$ is in~$\Psi_k$.
% \item For all~$t\in \NN$ the symmetric group~$\sym(t)$ is in~$\Psi_k$.

% \item If~$\Delta$ and~$\Delta'$ is in~$\Psi_k$ then the direct product~$\Delta\times \Delta'$ is in~$\Psi_k$.
% \item If~$\Delta$ and~$\Delta'$ is in~$\Psi_k$ then the wreath product~$\Delta\wr \Delta'$ is in~$\Psi_k$
% %\item If~$\Delta$ is in~$\Psi_k$ then~$\Delta\wr S_t$ is in~$\Psi_k$ for every~$t\in \mathbb{N}$.

% %\item If~$\Delta$ is in~$\Psi_k$ then for every subgroup~$\Lambda$ of~$S_k$ the group $\Delta\wr \Lambda$ is in~$\Psi_k$.

% \end{itemize}



\begin{theo}\label{theo:autG}
Every automorphism group of a graph of tree width at most~$k$ is in~$\Psi_k$.
\end{theo}

\begin{proof}
 Let~$G$ be a graph of tree width at most~$k$.  If~$G$ is not
  connected then the automorphism group is the direct product of
  wreath products of the automorphism groups of the components with
  symmetric groups. We can thus assume
  that~$G$ is connected.

  Consider the tree decomposition~$(T,\beta)$ of
  the~$k$-improvement~$G^k$ described in Theorem~\ref{theo:cliqueDecomposition}.
  Since the decomposition is automorphism-invariant we
  have~$\Aut(G) = \Aut(G,(T,\beta))$.

  We show the following statement by induction: If~$G$ is a graph with
  a tree decomposition~$(T,\beta)$ satisfying the properties of
  \cref{theo:cliqueDecomposition} and~$S\subseteq \beta(t)$ is a subset of
  the root bag, then~$\Theta =\Aut(G,(T,\beta))_{(S)}$, the point-wise stabilizer
  of~$S$, is in~$\Psi_k$.

First note that the root bag~$t$ of the decomposition is invariant
under~$\Theta$. Consequently, there is an induced homomorphism~$h$
from~$\Theta$ to~$\Theta|_{\beta(t)}$. Note that~$\Theta|_{\beta(t)}$
is a subgroup of $\aut(G[\beta(t)])$
which again is a subgroup of
$\aut(G^k[\beta(t)])$.
By \Cref{lem:imp}(2) the improvement $G^k$
again has tree width at most $k$
and therefore $\Theta|_{\beta(t)}\in \Phi_k^{\leq}$.

Consider the kernel~$\Delta$ of~$h$, the set of automorphism in~$\Theta$ that fix all vertices in~$\beta(t)$. 
Then~$\Theta$ is the wreath product of~$\Delta$ and~$\Theta|_{\beta(t)}$.

Suppose~$t_1,\ldots,t_\ell$ are the children of the root of~$T$. Let~$T_i$ be the decomposition of~$T$ below~$t_i$, and let~$G_i$ be the graph induced by the vertices that appear in bags of~$T_i$.
Call two children~$t_i,t_j$ of~$t$ equivalent, if~$t_i$ and~$t_j$ have the same
adhesion set~$S_i=S_j$ towards~$t$ and there is an isomorphism
from~$(G_i,(T_i,\beta|_{V(T_i)}))$ to~$(G_j,(T_j,\beta|_{V(T_j)}))$ that fixes all vertices in~$S_i$. Let~$r_1,\ldots,r_m$ be the equivalence classes with respect to this relation.

The group~$\Delta$ decomposes naturally into the direct product~$\Delta_1\times\Delta_2\times\ldots \times \Delta_m$ where each~$\Delta_j$ is the group of automorphism fixing~$\beta(t)$ and fixing all vertices outside the equivalence class~$r_j$.

If~$t^j_1,\ldots,t^j_{|r_j|}$ are the children of~$t$ in~$r_j$ then~$\Delta_j$
is the wreath product
of~$\aut(G_{t^j_1},(T_{t^j_1},\beta|_{V(T_{t^j_1})}))_{(S_{t^j_1})}$ with the
symmetric group~$\sym(|r_j|)$.
The group~$\aut(G_{t^j_1},(T_{t^j_1},\beta|_{V(T_{t^j_1})}))_{(S_{t^j_1})}$ is in~$\Psi_k$ by induction on the size of~$T$, which finishes the proof.
\end{proof}


Let us now turn to studying the groups in $\Phi^\le_k$. The results of
the previous section yield the following lemma.

\begin{lem}\label{lem:gammak}
  Let $G$ be a $k$-basic graph of tree width at most $k$.  Let
  $v\in V(G)$ be a vertex with degree at most $k$ in $G$.
  Then~$\aut(G)_v$, the group of automorphism of $G$ that fix $v$, is
  in $\Gammak$.
\end{lem}

\begin{proof}
By \Cref{theo:labelDecomposition} there is a mapping $f$
that assigns every $(G,v)$ a coset-labeled tree decomposition
$(T,\beta,\alpha)$ in an isomorphism invariant way.
The automorphism of $(T,\beta,\alpha)$, written $\aut(T,\beta,\alpha)$, are all
$\sigma\in\sym(V(G))$ such that $(T,\beta,\alpha)^\sigma:=(T,t\mapsto
\beta(t)^\sigma,t\mapsto\alpha(t)^\sigma)$ equals $(T,\beta,\alpha)$ up to
a renaming of the nodes in $V(T)$.

Our first claim is that $\aut(G,v)$ is a subgroup of $\aut(T,\beta,\alpha)$.
Let $\sigma\in\aut(G,v)$ be an arbitrary automorphism.
The construction of $(T,\beta,\alpha)$
from $(G,v)$ is isomorphism-invariant and therefore
$\sigma\in\aut(T,\beta,\alpha)$. More formally,
$(T,\beta,\alpha)^\sigma=f(G,v)^\sigma=f(G^\sigma,v^\sigma)=
f(G,v)=(T,\beta,\alpha)$ holds for any $\sigma\in\aut(G,v)$.
This proves the first claim.

Since $\aut(G,v)\leq\aut(T,\beta,\alpha)$ and $\Gammak$ is closed
under taking subgroups, it remains to show $\aut(T,\beta,\alpha)\in\Gammak$.
We proceed by induction on the number of nodes $n=|T|$ of $T$.

For $n=1$ every automorphism $\sigma$ fixing~$v$
%satisfies $\alpha^\sigma=\alpha$.
preserves $\alpha$.
Since there is only one $t\in T$
we conclude $\alpha(t)^\sigma=\alpha(t)$ or equivalently
$\aut(T,\beta,\alpha)\leq \Delta$, where we write
$\alpha(t)=\Delta\pi$. Now $\alpha(t)\in\gammak$ implies
$\aut(T,\beta,\alpha)\in\Gammak$.

Assume $n>1$ and let $t\in T$ be the root.
We
define a group homomorphism $h:\aut(T,\beta,\alpha)\to\sym(\beta(t))$ by the restriction of $\aut(T,\beta,\alpha)$ to $\beta(t)$. This homomorphism is well defined since~$\beta(t)$ is invariant under automorphisms.
Analogous to the base case one can show that the image of $h$
is in $\Gammak$. 

In general, for a group $\Theta$ and a normal subgroup
$N\trianglelefteq\Theta$
every composition factor of
$\Theta$ is a composition factor
of $N$ or a composition factor of the factor group $\Theta/N$.
%of a group in $\Gammak$ by a group in $\Gammak$ is a group that itself is in
% $\Gammak$,
Therefore, it suffices to show that the kernel of $h$, i.e., the set of
automorphism that fix the root bag pointwise, is in $\Gammak$.
The kernel of $h$ permutes the child-bags of $t$ with common adhesion sets.
Since the direct product of groups in $\Gammak$ is a group that is also in
$\Gammak$, we can restrict our attention to sets of children whose corresponding
subtrees have same adhesion set to the root bag.
Let $\Phi_1,\ldots,\Phi_r$ be the automorphism groups of subtrees rooted at
children of $t$ that all have the same adhesion set.
Notice that by Property \ref{i:4} of our coset-labeled tree decomposition
the number of children of $t$ with common adhesion set is bounded by $k$.

We can define a natural homomorphism into the permutation
group~$\{1,\ldots,r\}$ by considering the permutation of the children. With
similar arguments to before we conclude that it suffices to show the group of
automorphisms fixing the child-decompositions in~$\Gammak$. It thus suffices
to show that each group~$\Phi_i$ is in~$\Gammak$. Since~$\Phi_i$ is the automorphism group of some coset-labeled tree decomposition~$(T_i,\beta_i,\alpha_i)$ that is a subdecomposition of~$(T,\beta,\alpha)$, by induction hypothesis $\Phi_i\in\Gammak$ for each $i\in[r]$.
We conclude that $\aut(T,\beta,\alpha)\in\Gammak$.
\end{proof}

For a permutation~$\gamma\in \Sym(\Omega)$ we denote by~$\fix(\gamma)\coloneqq \{v\in \Omega\mid v^\gamma=v\}$ the set of points fixed by~$\gamma$. For a set of permutations~$S\subseteq \Sym(\Omega)$ we define~$\fix(S)\coloneqq \bigcap_{\gamma\in S}\fix(\gamma)$ as the points fixed by all elements in~$S$.


\begin{lem}\label{lem:order:p:fix:clique}
  For $k\geq 1$, let $G$ be a $k$-basic graph and
  let~$p> k$ be a prime.
  \begin{enumerate}
   \item If~$\gamma\in \Aut(G)$ has order~$p$ then~$\fix(\gamma)$ is a clique.
  \item If~$\gamma,\gamma'\in \Aut(G)$ commute and both have order~$p$ then~$\fix(\gamma)\cup \fix(\gamma')$ is a clique.
  
%  \item If~$\Gamma\leq  \Aut(G)$ is simple group that is not
%  isomorphic to a subgroup of~$\Sym(k-1)$ then there is a
%  connected~$\Gamma$-invariant subgraph~$G'$ of~$G$ on which the
%  induced action of~$\Gamma$ is fixed-point free. Moreover,~$\Aut(G)$
%  contains~$\Gamma^2$ as a subgroup or~$\fix(\Gamma)$ is not a
%  separator.\martin{Teil (3) sollte für meinen Geschmack ein separates
%    Lemma sein.}
  
 \end{enumerate}
%  ~$p\geq k$ the set of all vertices in~$V(G)$ that are fixed by some element in~$\Aut(G)$ of order~$p$ forms a clique.
   %  Suppose~$\Aut(G)$ has a an element~$g$ of prime order~$p\geq k$. Then the fixed points of~$g$ form a clique.
\end{lem}

\begin{proof}
%For the first part let~$\Gamma\leq  \Aut(G)$ be a group not not isomorphic to a subgroup of~$\Sym(\{1,\ldots,n-1\})$.
%let~$v\in V(G)$ be a vertex that is not fixed by~$\Gamma$. 
%Note first that the group induced by~$\Gamma$ on the orbit of~$v$ is isomorphic to~$\Gamma$, since~$\Gamma$ is simple.
%The assumption thus implies that the orbit of~$v$ under~$\Gamma$ has at least~$k$ elements.
%
%
%Consider~$C_v$, the connected component of~$G[V-\fix(\Gamma)]$ containing~$v$ and consider~$N\coloneqq N(C_v)\cap \fix(\Gamma)$, the set of vertices in~$\fix(\Gamma)$ that have a neighbor in~$C_v$.
%
%It suffices to show that~$N$ is a clique, since this implies that~$\fix(\Gamma) =N$.
%
%We show that every two vertices~$u$ and~$u'$ of~$N$ are adjacent. Let~$P$ be a shortest path from~$u$ to~$u'$ such that all internal vertices of~$P$ are in~$C_v$. Consider the set of edges~$P^{\Gamma}$.
%We claim that~$u$ and~$u'$ cannot be separated by at most~$k-1$ vertices.
%\ipascal{Don't know how to proceed from here? Halls theorem?}
Let~$\gamma\in \Aut(G)$ be an element of order~$p$.
We argue that the set~$F_\gamma\coloneqq \fix(\gamma)$ is a clique.
Let~$v$ be a vertex not fixed by~$\gamma$, i.e., 
$v\nin F_\gamma$.
Consider~$C_v$, the connected component of~$G[V\setminus F_\gamma]$
containing~$v$.

We claim that~$N(C_v)\subseteq F_\gamma$ is a clique. Let $u, u'\in N(C_v)$
and
let~$P$ be a shortest path from~$u$ to~$u'$ such that all internal vertices of~$P$ are in~$C_v$. For~$i\in \mathbb{N}$ the paths~$P$ and~$P^{(\gamma^i)}$ are internally vertex disjoint since~$P$ is a shortest path and no vertex in~$P$ is fixed under~$\gamma^i$.
We conclude that there are at least~$p> k$ internally vertex disjoint paths
between~$u$ and~$u'$. Thus, since~$G$ is~$k$-improved,~$u$ and~$u'$ must be
adjacent. This proves the claim that $N(C_v)$ is clique.

Since $N(C_v)$ separates $F_\gamma\setminus N(C_v)$ from $v$ and $G$ has no
separating cliques, it follows that $N(C_v)=F_\gamma$. This proves
Assertion (1).



To prove (2), suppose that~$\gamma'\in \Aut(G)$ is a second element of
order~$p$ that commutes with~$\gamma$. Let~$F_{\gamma'}\coloneqq \fix(\gamma')$ be
the elements fixed by~$\gamma'$. By (1), $F_{\gamma'}$ is clique.
It suffices to show that every vertex~$u$ in~$F_\gamma\setminus F_{\gamma'}$ is adjacent to every vertex~$w$ in~$F_{\gamma'}\setminus F_{\gamma}$.

Since~$\gamma$ and~$\gamma'$ commute, the set~$F_{\gamma'}\setminus F_{\gamma}$ is invariant under~$\gamma$. Let~$P$ be a shortest path from~$u$ to~$w$. For~$i\in\mathbb{N}$, we know that~$P^{(\gamma^i)}$ is a path from~$u$ to~$w^{(\gamma^i)}\in F_{\gamma'}\setminus F_{\gamma}$.
The paths~$P,P^{ \gamma^1}, \ldots,P^{(\gamma^{p-1})}$ form a set
of~$p> k$ internally vertex disjoint path all ending in distinct
endpoints $w_0,\ldots,w_{p-1}$, respectively. We have $w_0$, and all
$w_i$ are adjacent to $w$, because they are elements of the clique
$F_{\gamma'}$. Hence there are $p$ mutually disjoint paths from $u$ to
$w$. As $G$ is $k$-improved, it follows
that~$u$ and~$w$ are adjacent.
%
%For the third part 
%note that if the graph~$G -\fix(\Gamma)$ only has one component then
%the implications of the lemma hold.  Thus assume the graph has a least
%2 components.  Consider the induced action of~$\Gamma$ on the set of
%connected components of this graph. If this action is trivial then
%each component is a connected $\Gamma$-invariant subgraph of~$G$ and
%since~$\Gamma$ is simple,
%\martin{Warum brauchst Du hier simple?}
%the induced action of~$\Gamma$ on each
%component is fixed point free.
%Moreover, since $\Gamma$ is simple the
%induced action on each component is isomorphic to $\Gamma$,  and as
%there are at least two connected components, it follows that
%$\Gamma^2\le\Aut(G)$.\martin{Habe es etwas ausführlicher
%  geschrieben. Das Argumnet das $\Gamma^2\le\Aut(G)$ müsste für meine
%  Geschmack fast noch ausfürlicher sein.}
%
%If on the other hand~$\Gamma$ permuted
%the components of~$G -\fix(\Gamma)$ then, since~$\Gamma$ is simple the
%induced action of~$\Gamma$ on the components must be isomorphic
%to~$\Gamma$ as a permutation group. It follows from the assumption
%that there are at least~$k$ components~$C_1,\ldots,C_k$ that can be
%pairwise mapped to each other under~$\Gamma$. This implies
%that~$N(C_1)\cap \fix(\Gamma)$ is a clique, which contradicts $G$
%having no clique separator.
\end{proof}



%\begin{lem}
% For $k\geq 2$, let $G$ be a $k$-improved graph that is connected
%  and does not have any separating cliques. Let~$p\geq k$ be a prime.
%
%If~$\Gamma\leq  \Aut(G)$ is simple group then~$V(G)\setminus \fix(\Gamma)$ is connected or~$\Aut(G)$ contains a symmetric group that has a subgroup isomorphic to~$\Gamma$.
%\end{lem}
   
   
We will use the contraction lemma of
Babai~\cite{MR0316298}.
\begin{lem}[Contraction Lemma~\cite{MR0316298}]\label{theo:contractionlemma}
If~$\Gamma$ is a semiregular subgroup of the automorphism group of a graph~$G$ (i.e., the only element of~$\Gamma$ that has fixed points is the identity) then~$G$ has a minor isomorphic to a Cayley graph of~$\Gamma$.
\end{lem}

\begin{lem}\label{lem:minor}
  For $k\geq 1$, let $G$ be a
non-complete $k$-basic graph.
%  Suppose~$\Aut(G)$ has a point-stabilizer~$\Aut(G)_v$ such that~$p\nmid |\Aut(G)_v|$ for an odd prime~$p$.
   If for a prime~$p> k$,  the group $\mathbb{Z}_p^2$ is isomorphic to a
   subgroup of~$\Aut(G)$ then~$G$ has the~$p\times p$ toroidal grid~(i.e., $C_n
   \mathbin{\square} C_n$) as a minor.
\end{lem}

\begin{proof}
Let~$\Gamma$ be a subgroup of~$\Aut(G)$ isomorphic
to~$\mathbb{Z}_p^2$.
Let~$X\coloneqq V(G)\setminus \bigcup_{\gamma\in
  \Gamma} \fix(\gamma)$ be the set of vertices not fixed by any vertex
in~$\Gamma$.
Since $\Gamma$ is Abelian \cref{lem:order:p:fix:clique} implies
that $\bigcup_{\gamma\in\Gamma} \fix(\gamma)$ is a clique.
By assumption $G$ is non-complete and does not have any separating
cliques and therefore~$X$ is nonempty and connected.
Thus,~$\Gamma$ acts semi-regularly on~$X$.
By the contraction lemma (\cref{theo:contractionlemma}),~$X$ has a minor that is a Cayley graph of~$\mathbb{Z}_p^2$. We can assume that the Cayley graph is with respect to a minimal generating set~$\gamma_1,\gamma_2$. 
It suffices now to observe that the Cayley graph of~$\mathbb{Z}_p^2$ with respect to a generating set~$\gamma_1,\gamma_2$ is the toroidal grid.
\end{proof}


Since a $p\times p$-grid has tree width $p$ (a toroidal $p\times p$
even has tree width
either $2p-1$ or $2p-2$
\cite{Kiyomi:2016:TTG:2853242.2853625}),  the previous lemma shows
that the automorphism group of a $k$-basic graph of bounded treewdith
cannot contain $\mathbb{Z}_p^2$ as a subgroup.

% \begin{theo}[\cite{Kiyomi:2016:TTG:2853242.2853625}]\label{theo:toroidal}
% The tree width of the $p\times p$ toroidal grid is
% either $2p-1$ or $2p-2$ for any integer $p\geq 3$.
% \end{theo}
% 
% A combination of Theorem~\ref{theo:autG} and Lemma~\ref{lem:minor},
% together with other technical lemmas proved in the appendix, yields
% the following theorem. which is our main group theoretic result.

A group~$\Delta$ is a \emph{section} of a group~$\Gamma$ if there is a subgroup~$\Gamma'\leq \Gamma$ containing a normal subgroup~$N\trianglelefteq \Gamma'$ such that~$\Delta\cong \Gamma'/N$.
We say $\Gamma$ is $\Delta$-\emph{free}, if $\Delta$ is not a
section of $\Gamma$.
The next question is if $\ZZ_p^2$ could be a section of a group in $\Phi_k$
even for large primes $p>k$. It turns out that for $p>2$, the group $\ZZ_p^2$
has the very special property that it appears as a section, if and only if it is a subgroup.

\begin{lem}\label{lem:section}
If~$\ZZ_p^2$ is a section of a group~$\Gamma$ then~$\ZZ_p^2$ is also a
subgroup of~$\Gamma$ or~$p=2$ and the Sylow-2-groups of~$\Gamma$ are generalized quaternion groups.
\end{lem}

\begin{proof}
Let~$\gamma,\gamma'$ be lifts of two elements that generate~$\ZZ_p^2$.
By taking suitable powers, we can assume that the orders of~$\gamma$ and~$\gamma'$ are powers of~$p$.
By conjugating~$\gamma$ we can assume that they are contained in the
same~Sylow-$p$-group of~$\Gamma$.
We can thus assume that~$\Gamma$ is a~$p$-group.
All Abelian subgroups of~$\Gamma$ are cyclic, otherwise it
contains~$\ZZ_p^2$ and we are done.
By \cite{cartan2016homological}(Cartan, Eilenberg 1999, Theorem 11.6, p. 262)
we conclude that~$\Gamma$ is cyclic or a generalized quaternion group.
The former cannot be since~$\gamma$ and~$\gamma'$ are not powers of one another.
%Neither~$g$ nor~$g'$ is in the center, otherwise we are done.
%Let~$g''$ be an element of the center of the this means that~$g''$ is a power of~$g$ and of~$g$.
\end{proof}

\begin{theo}\label{theo:main-group}
Let $G$ be a graph of tree width $k\geq 2$.
%Let $M_k$ be the set of simple subgroups of $\sym(k)$.
Then every non-Abelian composition factor
of~$\aut(G)$ is alternating or $\ZZ_p^2$-free for all primes $p> k$.
\end{theo}

\begin{proof}
\Cref{theo:autG} shows that $\aut(G)\in\Psi_k$.
By definition of $\Psi_k$ the composition factors of any $\Delta\in\Psi_k$ are
isomorphic to a composition factor of of a member in:
$\Phi_k^{\leq}$ or $\sym(t)$ for some $t\in\NN$.
The composition factors of $\sym(t)$ are alternating.
So we are left to prove the statement for $\Phi_k^{\leq}$ groups.
Let $\Delta\in\Phi_k^{\leq}$.
Then there is $k$-basic graph $G$ of tree width at most $k$
such that $\Delta$ is isomorphic to a subgroup of $\aut(G)$.
Assume for contradiction that
$\Delta$ contains $\ZZ_p^2$ as a composition factor.
Then $\Aut(G)$ contains $\ZZ_p^2$ as a section.
By \cref{lem:section} the group $\aut(G)$ also contains $\ZZ_p^2$ as a
subgroup.
Then by \cref{lem:minor} the graph $G$ contains the
$p\times p$ toroidal grid as a minor or $G$ is the complete graph.
If $G$ has the $p\times p$ toroidal grid as a minor, then
the tree width of $G$ is at least $2p-2>k $
which is a contradiction.
If $G$ is complete, then $\ZZ_p^2$ is a subgroup of
the symmetric group on the vertex set.
In this case the number of vertices is at least $2p$,
but the complete graph on $2p$ vertices has tree width $2p-1>k$
which is again a contradiction.
\end{proof}


For completeness let us mention a converse to the statements presented.


\begin{lem}
Every group~$\Gamma \leq \sym(k)$ is isomorphic to the automorphism group of a
graph of tree width at most~$k$.
\end{lem}

The lemma can be shown by attaching suitable gadgets to a~$k$-clique.
We refer to~\cite{DBLP:conf/swat/OtachiS14}
(Lemma 16 in the arXiv version). 


%\subsection{Forbidden minors}
%
%\ipascal{Various errors and major gaps in this subsection.}
%
%We can use similar argument to the ones presented here to obtain results with regard to forbidden minors.
%
%
%\begin{lem}\label{lem:minor}
%  For $k\geq 1$, let $G$ be a $k$-complemented and
%non-complete graph that
%does not have any separating cliques.
%%  Suppose~$\Aut(G)$ has a point-stabilizer~$\Aut(G)_v$ such that~$p\nmid |\Aut(G)_v|$ for an odd prime~$p$.
%   If for a prime~$p\geq k$,  the group $\mathbb{Z}_p^3$ is isomorphic to a
%   subgroup of~$\Aut(G)$ then~$G$ has the complete graph~$K_p$ as a minor.
%\end{lem}
%
%
%
%\begin{lem}
%If~$G$ contains no~$K_k$ minor then the~$k$-complemented graph~$G^k$ contains no~$f(k)$-clique. \ipascal{Is something like this true?}
%\end{lem}
%
%
%
%\begin{cor}
%Let~$\Gamma$ be a finite simple group containing~$\mathbb{Z}_p^3$ as a subgroup. If~$\Aut(G) = \Gamma$ for some graph~$G$ then~$G$ contains~$K_p$ as a minor.
%\end{cor}
%
%\begin{proof}
%With arguments analogous to the ones in Theorem~\ref{theo:autG} we conclude that it suffices to consider graphs whose~$k$-complemented graphs are clique-separator free.
%\end{proof}
%This improves a previous result of Babai in two directions. 
%It drastically improves from exponential to linear, while we also have a linear lower bound. 
%It also talks about subgroups of~$k$ complemented graphs and not just subgroups of simple groups.
%
%
%
%\ipascal{For embeddable graphs Babai has various results that describe which kinds of~$\mathbb{Z}_p$ can be realized. We should probably reference some here.}
%\ipascal{Similar results can be said about minor closed graphs classes.}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

